First Large Scale Production of Low Radioactivity Argon From Underground Sources

We report on the first large-scale production of low radioactivity argon from underground gas wells. Low radioactivity argon is of general interest, in particular for the construction of large scale WIMP dark matter searches and detectors of reactor neutrinos for non-proliferation efforts. Atmospheric argon has an activity of about 1 Bq/kg from the decays of 39Ar; the concentration of 39Ar in the underground argon we are collecting is at least a factor of 100 lower than this value. The argon is collected from a stream of gas from a CO2 well in southwestern Colorado with a Vacuum Pressure Swing Adsorption (VPSA) plant. The gas from the well contains argon at a concentration of 400-600 ppm, and the VPSA plant produces an output stream with an argon concentration at the level of 30,000-50,000 ppm (3-5%) in a single pass. This gas is sent for further processing to Fermilab where it is purified by cryogenic distillation. The argon production rate is presently 0.5 kg/day.

==> distillation_paper/authorslist.tex <==
\author[princeton]{H. O.~Back\corref{cor1}}
\author[fnal]{T.~Alexander}
\author[augustana]{A.~Alton}
%\author[princeton]{F.~Calaprice}
\author[princeton]{C.~Condon}
\author[princeton]{E.~de Haas}
%\author[snolab]{R.~Ford}
\author[princeton]{C.~Galbiati}
\author[princeton]{A.~Goretti}
%\author[princeton]{L.~Grandi}
\author[princeton]{T.~Hohmann}
\author[princeton]{An.~Ianni}
\author[fnal]{C.~Kendziora}
\author[princeton]{B.~Loer\fnref{fn1}}
%\author[princeton]{P.~Meyers}
\author[fnal]{D.~Montanari}
\author[princeton]{P.~Mosteiro}
%\author[princeton]{A.~Nelson}
%\author[umass]{A.~Pocar}
\author[fnal]{S.~Pordes}

\cortext[cor1]{Corresponding author. {email: hback@fnal.gov} \\{Tel.: +1-630-840-2218}, {fax +1-630-840-4263} 
\\{address: Fermilab MS351, P.O. Box 500, Batavia, IL 60510}}
\fntext[fn1]{Now at Fermi National Accelerator Laboratory}

\address[princeton]{Department of Physics, Princeton University, Jadwin Hall, Princeton, NJ 08544}
\address[fnal]{Fermi National Accelerator Laboratory, P.O.~Box 500, Batavia, IL 60510}
%\address[snolab]{SNOLAB, 1039 Regional Road 24, Creighton Mine \#9, Lively, ON, Canada, P3Y 1N2}
%\address[umass]{Department of Physics, 1126 Lederle Graduate Research Tower (LGRT), University of Massachusetts, Amherst, MA 01003}
\address[augustana]{Augustana College, Physics Department, 2001 South Summit Ave., Sioux Falls, SD 57197}


==> distillation_paper/bibliography.tex <==
\begin{thebibliography}{99}
\bibitem{Loosli1983}
 H.H.~Loosli, Earth Plan.~Sci.~Lett.~\textbf{63}, 51 (1983).
\bibitem{Benetti2007}
 P.~Benetti et.~al. (WARP Collaboration), Nucl.~Instr.~Meth.~A \textbf{574}, 83 (2007).
\bibitem{Back2012} 
 H.O.~Back et.~al. pre-pint arXiv:1204.6024.
\bibitem{Xu2012}
 J.~Xu et.~al. pre-print arXiv:1204.6011.
\bibitem{Arey1900}
 A.L.~Arey, \textit{Elementary Chemistry for High Schools and Academies} (The MacMillan Company, New York, 1900), p. 204
\bibitem{McCabe1976}
 W.L.~McCabe and J.C.~Smith, \textit{Unit Operations of Chemical Engineering}, (3rd Edition, McGraw-Hill 1976); Perry's Chemical Engineers' Handbook, (7th Edition, McGraw-Hill 1997)
\bibitem{Perry1997}
 Robert H.~Perry and Don W.~Green, \textit{Perry's Chemical Engineers' Handbook} (7th Edition, McGraw-Hill 1997)
\bibitem{Halvorsen1999}
 Ivar J.~Halvorsen and Sigurd Skogestad, \textit{Encyclopedia of Separation Science}, (Chapter 2, Academic Press Ltd. 1999)
\bibitem{SRSA}
 Operating Manual and Programming Reference, Models RGA100, RGA200, and RGA300 Residual Gas Analyzer, Stanford Research Systems, Sunnydale, CA, 2009
%\bibitem{CryomechA}
% Cryomech Al600 Cryorefrigerator

\end{thebibliography}

